A Deep Dive Into How Open-Source Project Maintainers Review and Resolve Bug Bounty Reports

Researchers have investigated the bug bounty ecosystem from the lens of platforms, programs, and bug hunters. Understanding the perspectives of bug bounty report reviewers, especially those who historically lack a security background and little to no funding for bug hunters, is currently understudied. In this paper, we primarily investigate the perspective of open-source software (OSS) maintainers who have used \texttt{huntr}, a bug bounty platform that pays bounties to bug hunters who find security bugs in GitHub projects and have had valid vulnerabilities patched as a result. We address this area by conducting three studies: identifying characteristics through a listing survey ($n_1=51$), their ranked importance with Likert-scale survey data ($n_2=90$), and conducting semi-structured interviews to dive deeper into real-world experiences ($n_3=17$). As a result, we categorize 40 identified characteristics into benefits, challenges, helpful features, and wanted features. We find that private disclosure and project visibility are the most important benefits, while hunters focused on money or CVEs and pressure to review are the most challenging to overcome. Surprisingly, lack of communication with bug hunters is the least challenging, and CVE creation support is the second-least helpful feature for OSS maintainers when reviewing bug bounty reports. We present recommendations to make the bug bounty review process more accommodating to open-source maintainers and identify areas for future work.

==> content/nocolor_table.tex <==
 \begin{table*}[th!]
 \centering
 \begin{adjustbox}{width=\textwidth,totalheight=4.95in}
 \begin{tabular}{crlrrl}
 \toprule
 %\midrule
 & \multicolumn{1}{r}{\textbf{Characteristic}} & \multicolumn{1}{l}{\textbf{Description}} & \multicolumn{1}{r}{\textbf{RW}} & \multicolumn{1}{r}{\textbf{L}} & \multicolumn{1}{l}{$\bm{\pi}$}\\
 \midrule
 \parbox[t]{3mm}{\multirow{10}{*}{\rotatebox[origin=c]{90}{\textbf{Benefits of BBR Review}}}}
   & \textbf{Private disclosure} & Confidential communication of vulnerabilities to project maintainers. & \cite{beretas2023analysis, subramanian2020marketplaces, kuehn2014insttitutional} & 4 & 0.155 \\
   &\textbf{Project visibility} & ``Many eyes'' are available to help review a project. & \cite{maillart2017eyes, alexopoulos2021vuln-reporters} & 13 & 0.142 \\
   & \textbf{Detailed reports} & Receiving thorough bug reports to help timely patching. & & 8 & 0.138 \\
   &\textbf{Improved security posture} & Overall project defense, minimizing vulnerability risks. & \cite{zhao2015web-vulns, walshe2022cvd, atefi2023chromium, maulani2023case-study, bhushan2022dynamics, hendrick2023openssf, wermke2022qual-OSSP, zhao2016crowdsourced} & 33 & 0.124 \\
   & \textbf{Learning opportunities} & The ability to learn about threats and mitigations. & \cite{akgul2023BBHperspectives, ellis2022bounty} & 18 & 0.100 \\
   &\textbf{Benefits OSS users \& trust} & Transparent handling of security issues builds trust with users. & \cite{wermke2022qual-OSSP} & 13 & 0.077 \\
   & \textbf{Delegated bounties} & Bounty payments come from and are handled by an external entity. & \cite{hou2023temporal, finifter2013vuln-rewards, akgul2023BBHperspectives} & 9 & 0.070 \\
   &\textbf{Efficient development} & Additional time to focus on other development aspects. & & 7 & 0.069 \\
   & \textbf{Outsourced work} & Outsourced red-teaming of OSS project and community involvement. & \cite{walshe2020empiricalBBPs} & 4 & 0.064 \\
   &\textbf{Networking opportunities} & The ability to obtain security expert input and build connections. & \cite{alexopoulos2021vuln-reporters, huang2016multiple, ellis2022bounty} & 12 & 0.061 \\
  \midrule
 \parbox[t]{3mm}{\multirow{12}{*}{\rotatebox[origin=c]{90}{\textbf{Challenges in BBR Review}}}}
   & \textbf{Diverted focus} & Hunters are focused on money or CVEs, not software security. & \cite{hou2023temporal, finifter2013vuln-rewards, laszka2016banish, maillart2017eyes, ellis2022bounty} & 12 & 0.141 \\
   &\textbf{Pressure to review} & Reporters pushing to get their findings approved fast. & & 12 & 0.113 \\
   & \textbf{Testing difficulties} & Difficulty creating test cases for applied fixes. & & 5 & 0.112 \\
   &\textbf{Overstated severity} & Dealing with reports that do not reflect the bug's true severity. & & 9 & 0.096 \\
   & \textbf{Low-quality or spam} & Dealing with low-quality or spam reports. & \cite{walshe2022cvd, sridhar2021hackerone, shafigh2021invalid, laszka2016banish, zhao2020control, zhao2016crowdsourced} & 22 & 0.094 \\
   &\textbf{Validating impact} & Evaluating the practical security impact of a report. & & 11 & 0.085 \\
   & \textbf{Finding a fix} & Issues with finding and implementing fixes. & & 7 & 0.079 \\
   &\textbf{Reproduction difficulties} & Challenging to reproduce reported bugs for effective understanding. & & 10 & 0.079 \\
   & \textbf{Time-consuming} & Reviewing bug bounty reports takes up a lot of time. & \cite{walshe2022cvd} & 10 & 0.066 \\
   &\textbf{Knowledge gaps} & Gaps in security knowledge hinder bug assessment and resolution. & \cite{hendrick2023openssf} & 10 & 0.054 \\
   & \textbf{Duplicate reports} & Dealing with multiple identical or similar bug reports. & \cite{nagwani2021slr-dupes, ellis2022bounty, zhao2016crowdsourced} & 6 & 0.043 \\
   &\textbf{Lack of communication} & Inadequate communication between reporters and maintainers. & \cite{maulani2023case-study, akgul2023BBHperspectives, li2022relational, ellis2022bounty} & 6 & 0.038 \\
 \midrule
   \parbox[t]{3mm}{\multirow{9}{*}{\rotatebox[origin=c]{90}{\textbf{Helpful Features}}}}
   & \textbf{Incentivized reporting} & Bug hunters receive points for reporting valid vulnerabilities. & & 4 & 0.167 \\
   &\textbf{Security metric calculations} & Assistance in calculating security metrics (e.g., CVSS score). & & 5 & 0.133 \\
   & \textbf{Feedback capabilities} & The ability to provide feedback and make report adjustments. & & 6 & 0.122 \\
   &\textbf{Reducing project costs} & The existence of financial incentives from an external entity. & \cite{walshe2020empiricalBBPs} & 12 & 0.121 \\
   & \textbf{Secure disclosure} & Receiving private bug reports and publishing them after patching. & \cite{beretas2023analysis, badash2021blockchain} & 15 & 0.118 \\
   &\textbf{Easy report management} & User-friendly interface and varied features to manage bug reports. & & 14 & 0.109 \\
   & \textbf{Communication system} & Comments and messaging are available during the review process. & \cite{maulani2023case-study} & 8 & 0.106 \\
   &\textbf{CVE creation support} & Streamlined and assisted process of creating CVEs. & & 8 & 0.069 \\
   & \textbf{CI/CD mapping} & Integrating basic CI/CD details into bug reports. & & 7 & 0.054 \\
  \midrule
   \parbox[t]{3mm}{\multirow{9}{*}{\rotatebox[origin=c]{90}{\textbf{Wanted Features}}}}
   &\textbf{Collaboration features} & The ability to request reviews from security experts or other maintainers. & \cite{maulani2023case-study} & 2 & 0.163 \\ 
   & \textbf{Reputation system} & Additional ways to measure and assign reputation to bug hunters. & \cite{ohare2020game} & 4 & 0.145 \\
   &\textbf{More financial incentives} & E.g., rewards for bug fixes, bonuses for high-quality reports. & \cite{hou2023temporal, finifter2013vuln-rewards, gersbach2023decentralized, ellis2022bounty} & 4 & 0.145 \\
   & \textbf{PoC requirement} & Reports will be required to include a working proof-of-concept (PoC). & & 10 & 0.106* \\
   &\textbf{Environmental features} & E.g., support for in-built code review, rich text comments. & & 5 & 0.106* \\
   & \textbf{More management features} & E.g., report sorting, the ability to link duplicate reports. & & 4 & 0.104 \\
  &\textbf{Security guide \& FAQs} & Guides for bug bounty understanding and security-related FAQs. & \cite{hendrick2023openssf} & 5 & 0.101 \\
  & \textbf{Third-party integrations} & \underline{Automated} integration of CI/CD features for additional awareness. & & 8 & 0.074 \\
  &\textbf{Scheduled disclosure} & The ability to schedule when the report will be disclosed. & & 2 & 0.056 \\
  \bottomrule
 \end{tabular}
 \end{adjustbox}
 \caption{40 characteristics identified from the listing survey study divided into four categories as a result of bug bounty report (\textbf{BBR}) review. Acronyms listed represent, respectively: existing related work (\textbf{RW}), the number of listing (\textbf{L}) survey study mentions, and worth estimates ($\bm{\pi}$), for ranking responses, from the Likert-scale survey study. * indicates a tie.}
    \label{tab:bigasstable}
 %\end{centering}
 \end{table*}
